Self-stabilising approximate clock synchronisation requires linear time

Synchronising the clocks of processes is a fundamental problem in distributed computing. We consider message-passing systems in which processes start in an arbitrary initial state (self-stabilisation) and up to $f$ processes may be non-transiently faulty. It is well known that synchronising clocks \emph{exactly} is at least as hard as consensus and requires $\Theta(f)$ time. In contrast, without self-stabilisation, clocks can be synchronised \emph{approximately} much faster, in time independent of the number of non-transient faults [Srikanth and Toueg, JACM 1987; Welch and Lynch, Inf. Comput. 1988]. In this work, we show that deterministic self-stabilising approximate clock synchronisation tasks require $\Omega(f)$ time to stabilise. This gives the first non-trivial time lower bound for these tasks, whose time complexity has remained open for over two decades [Dolev and Welch, JACM 2004; Dolev, F\"ugger, Schmid and Lenzen, JACM 2014]. In particular, this answers the open question whether self-stabilising approximate clock synchronisation tasks are as hard as consensus or as easy as approximate agreement [Lenzen and Rybicki, JACM 2019]. The results show that guaranteeing \emph{both} transient and non-transient fault-tolerance simultaneously is expensive even for approximate synchronisation tasks. The lower bounds hold in a very strong model: the faulty processes can only crash, the local clocks of processes have no clock drift, and the message delay is bounded and known to all processes. The proof is based on a combinatorial topological argument showing that no fast finite-state protocol can ensure that the clocks behave consistently across all executions. To our knowledge, this is the first use of topological arguments to prove time lower bounds in the self-stabilising setting.

==> figures/figures.tex <==
\RequirePackage{tikz}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{decorations.markings}


\newif\ifWrapArcHighlight
\newif\ifWrapArcValues
\newif\ifWrapArcCut
\newif\ifWrapCycleDirection
\newsavebox{\WrapCycleNumberBox}
\pgfkeys{
  /wraparc/.is family, /wraparc,
  first label/.initial=i,
  second label/.initial=j,
  shared label/.initial={\WrapArcOption{first label},\WrapArcOption{second label}},
  value 1/.initial={},
  value 2/.initial={q-1},
  value 3/.initial=0,
  value 4/.initial={},
  radius/.initial=2.5cm,
  span/.initial=120,
  node inset/.initial=15,
  padding/.initial=6pt,
  scale/.initial=1,
  cycle nodes/.initial=6,
  q/.style={cycle nodes=#1},
  cycle rotation/.initial=0,
  cycle node size/.initial=22pt,
  cycle selected size/.initial={\WrapArcOption{cycle node size}},
  show direction/.is if=WrapCycleDirection, show direction=true,
  direction radius/.initial={.55*\WrapArcOption{radius}},
  direction start/.initial={90-180/\WrapArcOption{cycle nodes}+\WrapArcOption{cycle rotation}},
  direction span/.initial=120,
  direction color/.initial={\WrapArcOption{arc color}},
  direction width/.initial={\WrapArcOption{arc width}},
  arc color/.initial=black!70,
  arc width/.initial=1.2pt,
  highlight arc/.is if=WrapArcHighlight, highlight arc=false,
  highlight color/.initial=orange!85!black,
  highlight width/.initial=3.5pt,
  node size/.initial=9pt,
  node color/.initial=black!70,
  node fill/.initial=white,
  node width/.initial=1.2pt,
  selected size/.initial={\WrapArcOption{node size}},
  selected width/.initial=2.4pt,
  selected fill/.initial=waAccent,
  selected text color/.initial=white,
  show cut/.is if=WrapArcCut, show cut=true,
  cut length/.initial=14mm,
  cut color/.initial=black!75,
  cut width/.initial=1.2pt,
  cut dash pattern/.initial={on 3pt off 3pt},
  label font/.initial=\large,
  label color/.initial=waAccent,
  label gap/.initial=4pt,
  show values/.is if=WrapArcValues, show values=true,
  value font/.initial=\large,
  value color/.initial=black!85,
  value gap/.initial=9pt,
  value position/.is choice,
  value position/auto/.code={\def\waValuePlacement{0}},
  value position/below/.code={\def\waValuePlacement{1}},
  value position/above/.code={\def\waValuePlacement{2}},
  value position=auto
}
\newcommand{\WrapArcOption}[1]{\pgfkeysvalueof{/wraparc/#1}}
\newcommand{\WrapArcSetup}[1]{\pgfkeys{/wraparc/.cd,#1}}

\definecolor{coBlue}{HTML}{005A8D}
\newif\ifClockOffsetReverse
\newif\ifClockOffsetDirected
\pgfkeys{
  /wraparc/start label/.initial=b,
  /wraparc/end label/.initial=a,
  /wraparc/offset label/.initial={},
  /wraparc/reverse offset label/.initial={},
  /wraparc/show reverse/.is if=ClockOffsetReverse, /wraparc/show reverse=true,
  /wraparc/offset inner radius/.initial={.6*\WrapArcOption{radius}},
  /wraparc/offset outer radius/.initial={\WrapArcOption{radius}+.5*\WrapArcOption{cycle node size}+5pt},
  /wraparc/offset margin/.initial=24,
  /wraparc/directed edges/.is if=ClockOffsetDirected, /wraparc/directed edges=false,
  /wraparc/offset label gap/.initial=2pt,
  /wraparc/offset color/.initial={\WrapArcOption{highlight color}},
  /wraparc/reverse color/.initial=coBlue,
  /wraparc/reverse curvature/.initial={\WrapArcOption{offset inner radius}},
  /wraparc/interior fill/.initial=white,
  /wraparc/interior text/.initial=waAccent,
  /wraparc/offset style/.initial={},
  /wraparc/edge arrow/.initial={Stealth[length=5pt,width=4.5pt]},
  /wraparc/path arrow/.initial={Stealth[length=6pt,width=7pt]},
  /wraparc/offset arrow/.initial={Stealth[length=5pt,width=4.5pt]}
}
\newcommand{\ClockOffsetCycle}[3][]{%
  \begingroup
  \WrapArcSetup{#1}%
  \pgfmathtruncatemacro{\coCount}{\WrapArcOption{cycle nodes}}%
  \ifnum\coCount<3
    \PackageError{ClockOffsetCycle}{A cycle needs at least 3 nodes}{}%
  \fi
  \foreach \k in {#2,#3}{%
    \ifnum\k<0 \PackageError{ClockOffsetCycle}{Endpoint index must be nonnegative}{}\fi
    \ifnum\k<\coCount\else
      \PackageError{ClockOffsetCycle}{Endpoint index must be less than cycle nodes}{}%
    \fi
  }%
  \colorlet{waAccent}{\WrapArcOption{highlight color}}%
  \pgfmathsetlengthmacro{\coRadius}{\WrapArcOption{radius}}%
  \pgfmathsetmacro{\coCutAngle}{90+\WrapArcOption{cycle rotation}}%
  \pgfmathsetmacro{\coStart}{\coCutAngle-180/\coCount}%
  \pgfmathsetmacro{\coStep}{360/\coCount}%
  \pgfmathtruncatemacro{\coLast}{\coCount-1}%
  \pgfmathsetmacro{\coGap}{deg((\WrapArcOption{cycle node size}/2+\WrapArcOption{node width}/2)/\coRadius)}%
  \pgfmathsetmacro{\coSelGap}{deg((\WrapArcOption{cycle selected size}/2+\WrapArcOption{selected width}/2)/\coRadius)}%
  \ifClockOffsetDirected
    \tikzset{co/edge tip/.style={-{\WrapArcOption{edge arrow}}},
      co/path tip/.style={-{\WrapArcOption{path arrow}}}}%
  \else
    \tikzset{co/edge tip/.style={},co/path tip/.style={}}%
    \def\coGap{0}\def\coSelGap{0}%
  \fi
  \pgfmathtruncatemacro{\coSteps}{mod(#3-#2+\coCount,\coCount)}%
  \pgfmathtruncatemacro{\coSteps}{\coSteps>\coCount/2 ? \coSteps-\coCount : \coSteps}%
  \pgfmathtruncatemacro{\coAbsSteps}{abs(\coSteps)}%
  \pgfmathtruncatemacro{\coDir}{\coSteps<0 ? -1 : 1}%
  \pgfmathsetmacro{\coFrom}{\coStart-\coStep*(#2)}%
  \pgfmathsetmacro{\coMid}{\coFrom-\coStep*\coSteps/2}%
  \pgfmathsetlengthmacro{\coCutInner}{\coRadius-\WrapArcOption{cut length}/2}%
  \pgfmathsetlengthmacro{\coCutOuter}{\coRadius+\WrapArcOption{cut length}/2}%
  \pgfmathsetlengthmacro{\coBound}{\coRadius+\WrapArcOption{padding}}%
  \pgfmathsetlengthmacro{\coInner}{\WrapArcOption{offset inner radius}}%
  \pgfmathsetlengthmacro{\coOuter}{\WrapArcOption{offset outer radius}}%
  \sbox{\WrapCycleNumberBox}{{\WrapArcOption{value font}$\mathbf{0123456789}$}}%
  \begin{tikzpicture}[
    scale=\WrapArcOption{scale},transform shape,line cap=round,baseline={(0,0)},
    co/offset/.style={\WrapArcOption{offset style}},
    co/edge/.style={draw=\WrapArcOption{arc color},line width=\WrapArcOption{arc width},
      co/edge tip},
    co/path/.style={draw=waAccent,line width=\WrapArcOption{highlight width},
      co/path tip},
    co/node/.style={circle,draw=\WrapArcOption{node color},
      fill=\WrapArcOption{node fill},line width=\WrapArcOption{node width},
      minimum size=\WrapArcOption{cycle node size},inner sep=1pt,
      font=\WrapArcOption{value font},text=\WrapArcOption{value color},
      align=center,text height=\ht\WrapCycleNumberBox,text depth=\dp\WrapCycleNumberBox},
    co/interior/.style={co/node,draw=waAccent,fill=\WrapArcOption{interior fill},text=\WrapArcOption{interior text},
      line width=\WrapArcOption{selected width}},
    co/selected/.style={co/node,draw=waAccent,fill=\WrapArcOption{selected fill},
      text=\WrapArcOption{selected text color},
      minimum size=\WrapArcOption{cycle selected size},line width=\WrapArcOption{selected width}},
    co/label/.style={font=\WrapArcOption{label font},text=\WrapArcOption{label color},
      inner sep=1pt,text height={},text depth={}}
  ]
    \path (-\coBound,-\coBound) rectangle (\coBound,\coBound);
    \ifWrapArcCut
      \draw[draw=\WrapArcOption{cut color},line width=\WrapArcOption{cut width},
        dash pattern/.expanded=\WrapArcOption{cut dash pattern}]
        (\coCutAngle:\coCutInner)--(\coCutAngle:\coCutOuter);
    \fi
    \foreach \k in {0,...,\coLast}{
      \pgfmathtruncatemacro{\coNext}{mod(\k+1,\coCount)}
      \def\coEndGap{\coGap}
      \ifnum\coNext=#2\relax\def\coEndGap{\coSelGap}\fi
      \ifnum\coNext=#3\relax\def\coEndGap{\coSelGap}\fi
      \pgfmathsetmacro{\coA}{\coStart-\coStep*\k}
      \draw[co/edge] (\coA:\coRadius)
        arc[start angle=\coA,delta angle=-\coStep+\coEndGap,radius=\coRadius];
    }
    \ifnum\coAbsSteps>0
      \foreach \s in {1,...,\coAbsSteps}{
        \pgfmathsetmacro{\coA}{\coFrom-\coDir*\coStep*(\s-1)}
        \def\coEndGap{\coGap}
        \ifnum\s=\coAbsSteps\relax\def\coEndGap{\coSelGap}\fi
        \draw[co/path] (\coA:\coRadius)
          arc[start angle=\coA,delta angle=-\coDir*(\coStep-\coEndGap),radius=\coRadius];
      }
      \pgfmathsetmacro{\coHalf}{\coStep*\coAbsSteps/2-\WrapArcOption{offset margin}}
      \pgfmathsetlengthmacro{\coRevRadius}{\WrapArcOption{reverse curvature}}
      \pgfmathsetlengthmacro{\coRevCentre}{\coOuter-\coRevRadius}
      \pgfmathsetmacro{\coRevHalf}{\coHalf*\coInner/\coRevRadius}
      \pgfmathsetlengthmacro{\coInnerText}{\coInner-\WrapArcOption{offset label gap}}
      \pgfmathsetlengthmacro{\coOuterText}{\coOuter+\WrapArcOption{offset label gap}}
      \pgfkeysgetvalue{/wraparc/offset label}{\coText}%
      \ifx\coText\empty
        \ifnum\coSteps>0 \def\coText{+\coSteps}\else\let\coText\coSteps\fi
      \fi
      \draw[co/offset,draw=\WrapArcOption{offset color},line width=\WrapArcOption{arc width},
        -{\WrapArcOption{offset arrow}}]
        (\coMid+\coDir*\coHalf:\coInner)
        arc[start angle=\coMid+\coDir*\coHalf,delta angle=-2*\coDir*\coHalf,radius=\coInner];
      \node[co/offset,co/label,text=\WrapArcOption{offset color},anchor=\coMid]
        at (\coMid:\coInnerText) {$\coText$};
      \ifClockOffsetReverse
        \pgfkeysgetvalue{/wraparc/reverse offset label}{\coText}%
        \ifx\coText\empty
          \pgfmathtruncatemacro{\coNeg}{-\coSteps}%
          \ifnum\coNeg>0 \def\coText{+\coNeg}\else\let\coText\coNeg\fi
        \fi
        \draw[co/offset,draw=\WrapArcOption{reverse color},line width=\WrapArcOption{arc width},
          -{\WrapArcOption{offset arrow}}]
          [shift={(\coMid:\coRevCentre)}] (\coMid-\coDir*\coRevHalf:\coRevRadius)
          arc[start angle=\coMid-\coDir*\coRevHalf,delta angle=2*\coDir*\coRevHalf,radius=\coRevRadius];
        \pgfmathsetmacro{\coOpposite}{\coMid+180}
        \node[co/offset,co/label,text=\WrapArcOption{reverse color},anchor=\coOpposite]
          at (\coMid:\coOuterText) {$\coText$};
      \fi
    \fi
    \foreach \k in {0,...,\coLast}{
      \pgfmathsetmacro{\coAngle}{\coStart-\coStep*\k}
      \def\coStyle{co/node}
      \pgfmathtruncatemacro{\coPos}{mod(\coDir*(\k-#2)+2*\coCount,\coCount)}
      \ifnum\coPos>0 \ifnum\coPos<\coAbsSteps\relax\def\coStyle{co/interior}\fi\fi
      \def\coName{}
      \ifnum\k=#2\relax
        \def\coStyle{co/selected}\def\coName{\WrapArcOption{start label}}
      \fi
      \ifnum\k=#3\relax
        \def\coStyle{co/selected}\def\coName{\WrapArcOption{end label}}
        \ifnum#2=#3\relax\def\coName{\WrapArcOption{shared label}}\fi
      \fi
      \tikzset{co/name label/.style={}}
      \ifx\coName\empty\else
        \tikzset{co/name label/.style={label={
          [co/label,label distance=\WrapArcOption{label gap}]\coAngle:{$\coName$}}}}
      \fi
      \node[\coStyle,co/name label] at (\coAngle:\coRadius)
        {\ifWrapArcValues$\mathbf{\k}$\fi};
    }
  \end{tikzpicture}%
  \endgroup
}

\newif\ifOffsetSquareLifts
\pgfkeys{
  /offsetsquare/.is family, /offsetsquare,
  show lifts/.is if=OffsetSquareLifts, show lifts=true,
  q/.initial=5,
  width/.initial=3.2cm,
  height/.initial=1.9cm,
  advance color/.initial=black!70,
  offset color/.initial={orange!85!black},
  note color/.initial=black!50,
  corner 1/.initial={}, corner 2/.initial={}, corner 3/.initial={}, corner 4/.initial={},
  note 1/.initial={}, note 2/.initial={}, note 3/.initial={}, note 4/.initial={},
  advance i/.initial={}, advance j/.initial={},
  offset T/.initial={}, offset T+1/.initial={},
  first process/.initial={process $i$},
  second process/.initial={process $j$},
  first round/.initial={round $T$},
  second round/.initial={round $T+1$},
  process gap/.initial=1.6cm,
  round gap/.initial=.8cm,
  baseline/.initial={(current bounding box.center)},
  tikz/.initial={}
}
\newcommand{\OffsetSquareOption}[1]{\pgfkeysvalueof{/offsetsquare/#1}}
\newcommand{\OffsetSquareSigned}[1]{\ifnum#1>0 +\fi#1}
\newcommand{\OffsetSquareText}[2]{%
  \pgfkeysgetvalue{/offsetsquare/#1}{\osValue}%
  \ifx\osValue\empty #2\else\osValue\fi}
\newcommand{\OffsetSquare}[5][]{%
  \begingroup
  \pgfkeys{/offsetsquare/.cd,#1}%
  \pgfmathtruncatemacro{\osQ}{\OffsetSquareOption{q}}%
  \pgfmathtruncatemacro{\osOutA}{mod(mod(#2,\osQ)+\osQ,\osQ)}%
  \pgfmathtruncatemacro{\osOutB}{mod(mod(#3,\osQ)+\osQ,\osQ)}%
  \pgfmathtruncatemacro{\osOutC}{mod(mod(#4,\osQ)+\osQ,\osQ)}%
  \pgfmathtruncatemacro{\osOutD}{mod(mod(#5,\osQ)+\osQ,\osQ)}%
  \pgfmathtruncatemacro{\osAdvI}{#3-#2}%
  \pgfmathtruncatemacro{\osAdvJ}{#5-#4}%
  \pgfmathtruncatemacro{\osOffT}{#4-#2}%
  \pgfmathtruncatemacro{\osOffU}{#5-#3}%
  \begin{tikzpicture}[
    x=\OffsetSquareOption{width},y=\OffsetSquareOption{height},
    line cap=round,baseline/.expanded=\OffsetSquareOption{baseline},
    os/corner/.style={inner sep=3pt,font=\normalsize,minimum height=16pt},
    os/advance/.style={draw=\OffsetSquareOption{advance color},line width=1.2pt,
      -{Stealth[length=5pt,width=4.5pt]},shorten <=2pt,shorten >=2pt},
    os/offset/.style={draw=\OffsetSquareOption{offset color},line width=1.2pt,
      -{Stealth[length=5pt,width=4.5pt]},shorten <=1pt,shorten >=1pt},
    os/note/.style={font=\small,text=\OffsetSquareOption{note color},inner sep=1pt},
    os/axis/.style={font=\normalsize,inner sep=2pt},
    os/first/.style={},os/second/.style={},os/process label/.style={},
    os/advance i/.style={},os/advance j/.style={},
    os/offset label T/.style={},os/offset label T+1/.style={}
  ]
    \pgfkeysgetvalue{/offsetsquare/tikz}{\osTikz}%
    \expandafter\tikzset\expandafter{\osTikz}%
    \ifOffsetSquareLifts
      \def\osA{#2}\def\osB{#3}\def\osC{#4}\def\osD{#5}%
    \else
      \let\osA\osOutA\let\osB\osOutB\let\osC\osOutC\let\osD\osOutD
    \fi
    \node[os/corner,os/first] (a) at (0,1) {$\OffsetSquareText{corner 1}{\osA}$};
    \node[os/corner,os/first] (b) at (1,1) {$\OffsetSquareText{corner 2}{\osB}$};
    \node[os/corner,os/second] (c) at (0,0) {$\OffsetSquareText{corner 3}{\osC}$};
    \node[os/corner,os/second] (d) at (1,0) {$\OffsetSquareText{corner 4}{\osD}$};
    \draw[os/advance] (a) to[os/advance i] node[above,text=\OffsetSquareOption{advance color}]
      {$\OffsetSquareText{advance i}{\OffsetSquareSigned{\osAdvI}}$} (b);
    \draw[os/advance] (c) to[os/advance j] node[below,text=\OffsetSquareOption{advance color}]
      {$\OffsetSquareText{advance j}{\OffsetSquareSigned{\osAdvJ}}$} (d);
    \draw[os/offset] (a) -- node[left,text=\OffsetSquareOption{offset color},os/offset label T]
      {$\OffsetSquareText{offset T}{\OffsetSquareSigned{\osOffT}}$} (c);
    \draw[os/offset] (b) -- node[right,text=\OffsetSquareOption{offset color},os/offset label T+1]
      {$\OffsetSquareText{offset T+1}{\OffsetSquareSigned{\osOffU}}$} (d);
    \ifOffsetSquareLifts
    \node[os/note,anchor=south] at (a.north) {\OffsetSquareText{note 1}{(\osOutA)}};
    \node[os/note,anchor=south] at (b.north) {\OffsetSquareText{note 2}{(\osOutB)}};
    \node[os/note,anchor=north] at (c.south) {\OffsetSquareText{note 3}{(\osOutC)}};
    \node[os/note,anchor=north] at (d.south) {\OffsetSquareText{note 4}{(\osOutD)}};
    \fi
    \pgfkeysgetvalue{/offsetsquare/first process}{\osValue}%
    \ifx\osValue\empty\else
      \node[os/axis,os/process label,anchor=east] at ([xshift=-\OffsetSquareOption{process gap}]a.center) {\osValue};\fi
    \pgfkeysgetvalue{/offsetsquare/second process}{\osValue}%
    \ifx\osValue\empty\else
      \node[os/axis,os/process label,anchor=east] at ([xshift=-\OffsetSquareOption{process gap}]c.center) {\osValue};\fi
    \pgfkeysgetvalue{/offsetsquare/first round}{\osValue}%
    \ifx\osValue\empty\else
      \node[os/axis,anchor=base] at ([yshift=\OffsetSquareOption{round gap}]a.center) {\osValue};\fi
    \pgfkeysgetvalue{/offsetsquare/second round}{\osValue}%
    \ifx\osValue\empty\else
      \node[os/axis,anchor=base] at ([yshift=\OffsetSquareOption{round gap}]b.center) {\osValue};\fi
  \end{tikzpicture}%
  \endgroup
}

\newsavebox{\gcPanelA}
\newsavebox{\gcPanelB}
\newsavebox{\gcPanelC}
\newif\ifgcSquare
\newif\ifgcWinding
\definecolor{gcBlue}{HTML}{005A8D}
\definecolor{gcGreen}{HTML}{007A53}
\definecolor{gcPlum}{HTML}{9A3E6B}
\tikzset{
  gc/node/.style={rectangle,rounded corners=2.5pt,draw=white,line width=.7pt,
    minimum size=18pt,inner sep=1.5pt,text=white,font=\normalsize\bfseries,
    text height=1.6ex,text depth=0pt},
  gc/a/.style={fill=gcBlue},
  gc/b/.style={fill=gcGreen},
  gc/c/.style={fill=gcPlum},
  gc/face/.style={fill=gcBlue!12},
  gc/edge/.style={draw=black!40,line width=.9pt},
  gc/mid arrow/.style={postaction={decorate},decoration={markings,
    mark=at position .55 with {\arrow[#1]{Stealth[length=6.5pt,width=5.5pt]}}}},
  gc/oriented/.style={gc/mid arrow=black!85},
  gc/loop/.style={draw=orange!85!black,line width=2pt,gc/mid arrow=orange!85!black},
  gc/loop label/.style={font=\small,text=orange!85!black,inner sep=1pt},
  gc/legend box/.style={rectangle,rounded corners=2pt,minimum size=9pt,inner sep=0pt},
  gc/legend text/.style={anchor=west,font=\normalsize,inner sep=0pt,
    text height=1.5ex,text depth=.3ex},
}
\newcommand{\gcEdge}[6]{%
  \pgfmathtruncatemacro{\gcResidue}{mod(#6-#4+#1,#1)}%
  \ifnum\gcResidue=0
    \draw[gc/edge] (#3)--(#5);%
  \else\ifnum\gcResidue>#2
    \draw[gc/edge,gc/oriented] (#5)--(#3);%
  \else
    \draw[gc/edge,gc/oriented] (#3)--(#5);%
  \fi\fi
}
\newcommand{\GradientWindingComparisonFigure}[1][0.65]{%
  \begingroup\gcSquaretrue\gcWindingtrue\GradientComparisonFigure[#1]\endgroup}
\newcommand{\GradientComparisonFigure}[1][0.8]{%
  \begingroup
  \ifgcWinding
    \def\gcTop{2}\def\gcTopm{1}\def\gcAx{2.3cm}\def\gcAy{1.55cm}%
  \else
    \def\gcTop{2}\def\gcTopm{1}\def\gcAx{2cm}\def\gcAy{1.6cm}%
  \fi
  \sbox{\gcPanelA}{\begin{tikzpicture}[x=\gcAx,y=\gcAy,scale=#1,
      line cap=round,line join=round,baseline=(current bounding box.center)]
    \foreach \col in {0,...,3}{
      \foreach \row in {0,...,\gcTop}{
        \coordinate (gca-\col-\row) at (\col,\row);
      }
    }
    \foreach \col in {0,...,2}{
      \pgfmathtruncatemacro{\nextcol}{\col+1}
      \foreach \row in {0,...,\gcTopm}{
        \pgfmathtruncatemacro{\nextrow}{\row+1}
        \fill[gc/face] (gca-\col-\row)--(gca-\nextcol-\row)--(gca-\nextcol-\nextrow)--cycle;
        \fill[gc/face] (gca-\col-\row)--(gca-\col-\nextrow)--(gca-\nextcol-\nextrow)--cycle;
      }
    }
    \foreach \col in {0,...,3}{
      \pgfmathtruncatemacro{\gcOut}{mod(\col+2,4)}
      \foreach \row in {0,...,\gcTopm}{
        \pgfmathtruncatemacro{\nextrow}{\row+1}
        \gcEdge{4}{1}{gca-\col-\row}{\gcOut}{gca-\col-\nextrow}{\gcOut}
      }
    }
    \foreach \col in {0,...,2}{
      \pgfmathtruncatemacro{\nextcol}{\col+1}
      \pgfmathtruncatemacro{\gcOut}{mod(\col+2,4)}
      \pgfmathtruncatemacro{\gcNextOut}{mod(\col+3,4)}
      \foreach \row in {0,...,\gcTop}{
        \gcEdge{4}{1}{gca-\col-\row}{\gcOut}{gca-\nextcol-\row}{\gcNextOut}
      }
      \foreach \row in {0,...,\gcTopm}{
        \pgfmathtruncatemacro{\nextrow}{\row+1}
        \gcEdge{4}{1}{gca-\col-\row}{\gcOut}{gca-\nextcol-\nextrow}{\gcNextOut}
      }
    }
    \foreach \u/\v in {1-0/2-0,2-0/3-1,1-0/2-1,2-1/3-1}{
      \draw[gc/edge,gc/loop] (gca-\u)--(gca-\v);
    }
    \foreach \col in {0,...,3}{
      \pgfmathtruncatemacro{\gcOut}{mod(\col+2,4)}
      \foreach \row in {0,...,\gcTop}{
        \pgfmathtruncatemacro{\gcProcess}{mod(\col+\row,3)}
        \ifcase\gcProcess\def\gcStyle{gc/a}\or\def\gcStyle{gc/b}\or\def\gcStyle{gc/c}\fi
        \node[gc/node,\gcStyle] at (gca-\col-\row) {\gcOut};
      }
    }
  \end{tikzpicture}}%
  \sbox{\gcPanelB}{\begin{tikzpicture}[x=1.5cm,y=1.5cm,scale=#1,
      line cap=round,line join=round,baseline=(current bounding box.center)]
    \coordinate (gcb-0) at ( 0, .82);
    \coordinate (gcb-4) at (-.76,-.44);
    \coordinate (gcb-2) at ( .76,-.44);
    \coordinate (gcb-1) at ( 0, 2.05);
    \coordinate (gcb-5) at (-2.15,-1.10);
    \coordinate (gcb-3) at ( 2.15,-1.10);
    \foreach \u/\v/\w in {0/1/2,1/2/3,2/3/4,3/4/5,4/5/0,5/0/1}{
      \fill[gc/face] (gcb-\u)--(gcb-\v)--(gcb-\w)--cycle;
    }
    \foreach \u/\v in {4/2,2/0,0/4,5/3,3/1,1/5,0/1,2/1,2/3,4/3,4/5,5/0}{
      \gcEdge{6}{2}{gcb-\u}{\u}{gcb-\v}{\v}
    }
    \foreach \v/\p in {0/a,4/b,2/c,1/b,5/c,3/a}{
      \node[gc/node,gc/\p] at (gcb-\v) {\v};
    }
  \end{tikzpicture}}%
  \ifgcWinding
  \sbox{\gcPanelB}{\begin{tikzpicture}[x=1.5cm,y=1.5cm,scale=#1,
      line cap=round,line join=round,baseline=(current bounding box.center)]
    \foreach \k/\x/\y in {0/-1/1,1/1/1,2/1/-1,3/-1/-1}{
      \coordinate (gcw-i\k) at (.8*\x,.8*\y);
      \coordinate (gcw-o\k) at (1.72*\x,1.72*\y);
    }
    \foreach \u/\v/\w in {i0/o0/o1,i0/o3/o0,i0/i1/o1,i1/i2/o1,
        i2/o1/o2,i2/o2/o3,i2/i3/o3,i3/i0/o3}{
      \fill[gc/face] (gcw-\u)--(gcw-\v)--(gcw-\w)--cycle;
    }
    \foreach \u/\a/\v/\b in {o0/0/o1/1,o1/1/o2/2,o2/2/o3/3,o3/3/o0/0,
        i0/0/o0/0,i0/0/o1/1,i1/1/o1/1,i2/2/o1/1,
        i2/2/o2/2,i2/2/o3/3,i3/3/o3/3,i0/0/o3/3}{
      \gcEdge{4}{1}{gcw-\u}{\a}{gcw-\v}{\b}
    }
    \foreach \u/\v in {i0/i1,i1/i2,i2/i3,i3/i0}{
      \draw[gc/edge,gc/loop] (gcw-\u)--(gcw-\v);
    }
    \foreach \u/\o/\p in {i0/0/a,i1/1/b,i2/2/a,i3/3/b,o0/0/b,o1/1/c,o2/2/b,o3/3/c}{
      \node[gc/node,gc/\p] at (gcw-\u) {\o};
    }
  \end{tikzpicture}}%
  \fi
  \ifgcSquare\let\gcOuter\relax\else\let\gcOuter\hfil\fi
  \ifgcSquare
    \sbox{\gcPanelC}{\OffsetSquare[q=4,width=2.8cm,height=1.6cm,
      tikz={os/first/.style={gc/node,gc/a},os/second/.style={gc/node,gc/b},
        os/advance/.append style={dashed,draw=black!45,line width=.9pt},
        os/note/.append style={font=\normalsize},
        os/advance i/.style={bend left=40},os/advance j/.style={bend right=40},
        os/offset/.style={gc/edge,gc/oriented},
        os/offset label T/.style={anchor=south,rotate=90},
        os/offset label T+1/.style={anchor=north,rotate=90}},
      offset color=black,
      corner 1=\mathbf{3},corner 2=\mathbf{0},corner 3=\mathbf{0},corner 4=\mathbf{1},
      note color=black,
      note 1=$\prefix{y_i}$,note 2=$\suffix{y_i}$,
      note 3=$\prefix{y_j}$,note 4=$\suffix{y_j}$,
      offset T={\relax},offset T+1={\relax},%
      first process={},second process={},first round={},second round={}]{3}{4}{4}{5}}%
  \else
    \sbox{\gcPanelC}{}%
  \fi
  \sbox{\gcPanelA}{\vbox{%
    \hbox to \wd\gcPanelA{\hss\tikz[baseline=-.55ex]{%
      \node[gc/legend text,anchor=east] at (-.3,0) {processes};
      \foreach \p/\name/\x in {a/i/0,b/j/1,c/k/2}{
        \node[gc/legend box,gc/\p] at (\x,0) {};
        \node[gc/legend text] at (\x+.22,0) {$\name$};
      }}\hss}%
    \vskip 1.1em
    \hbox{\usebox{\gcPanelA}}}}%
  \centerline{\vbox{\hsize=\textwidth
    \hbox to \hsize{\gcOuter$\vcenter{\hbox{\usebox{\gcPanelA}}}$\hfil
      $\vcenter{\hbox{\usebox{\gcPanelB}}}$\hfil
      \ifgcSquare$\vcenter{\hbox{\usebox{\gcPanelC}}}$\gcOuter\fi}%
    \vskip .4em
    \hbox to \hsize{\normalsize\gcOuter\makebox[\wd\gcPanelA]{(a)}\hfil
      \makebox[\wd\gcPanelB]{(b)}\hfil
      \ifgcSquare\makebox[\wd\gcPanelC]{(c)}\gcOuter\fi}%
  }}%
  \endgroup
}

\definecolor{psBlue}{HTML}{005A8D}
\tikzset{
  ps/pulse/.style={line width=1.7pt,line cap=butt},
  ps/stable/.style={ps/pulse,draw=psBlue},
  ps/free/.style={ps/pulse,draw=black!38},
  ps/line/.style={draw=black!28,line width=.6pt},
  ps/wave/.style={fill=psBlue!10,rounded corners=2pt},
  ps/phase/.style={fill=black!5,rounded corners=2pt},
  ps/guide/.style={draw=black!35,line width=.4pt,densely dotted},
  ps/dim/.style={draw=black!75,line width=.6pt,
    {Stealth[length=4pt,width=3.5pt]}-{Stealth[length=4pt,width=3.5pt]}},
}
\tikzset{
  cc/free/.style={text=black!40},
  cc/stable/.style={text=psBlue},
  ps/stabline/.style={draw=black!55,line width=.6pt,dash pattern=on 2.5pt off 2pt},
}
\newcommand{\ccStableLabel}{counting}
\newcommand{\ccT}{4}
\newcommand{\ccLast}{10}%
\newcommand{\ccRow}[4]{%
  \foreach \v [count=\c from #3] in {#4}{
    \node[#2] at (\c,#1) {$\v$};
  }%
}
\newcommand{\ccPanel}[9]{%
  \begin{scope}[xshift=#1]
    \fill[ps/phase] (-.5,.5) rectangle (\ccT-.5,-3.5);
    \draw[ps/stabline] (\ccT-.5,.5)--(\ccT-.5,-4.05);
    \node[anchor=base,font=\small\bfseries,text=black!60] at ({(\ccT-1)/2},.78) {stabilisation};
    \node[anchor=base,font=\small\bfseries,text=psBlue] at ({(\ccT+\ccLast)/2},.78) {\ccStableLabel};
    \foreach \r/\p in {0/1,1/2,2/3,3/4}{
      \node[anchor=east] at (-.75,-\r) {$\p$};
    }
    \ccRow{0}{cc/free}{0}{#3}
    \ccRow{-1}{cc/free}{0}{#4}
    \ccRow{-2}{cc/free}{0}{#5}
    \ccRow{-3}{cc/free}{0}{#6}
    \draw[black!55,line width=.9pt,line cap=butt]
      (2,-3) +(-.17,-.17) -- +(.17,.17) +(-.17,.17) -- +(.17,-.17);
    \ccRow{0}{cc/stable}{\ccT}{#7}
    \ccRow{-1}{cc/stable}{\ccT}{#8}
    \ccRow{-2}{cc/stable}{\ccT}{#9}
    \draw[black!60,line width=.6pt,-{Stealth[length=4pt,width=3.5pt]}]
      (-.5,-4.05)--(\ccLast+1,-4.05);
    \node[anchor=east] at (-.75,-4.05) {$t$};
    \foreach \x in {0,...,\ccLast}{
      \draw[black!60,line width=.6pt] (\x,-4.05)--(\x,-4.17);
    }
    \node[below] at (0,-4.17) {$0$};
    \node[below] at (\ccT,-4.17) {$T$};
    \node at (\ccLast/2,-5.55) {#2};
  \end{scope}%
}
\newcommand{\CountingPulseFigure}[1][]{%
  \begin{tikzpicture}[x=.6cm,y=.6cm,line cap=round,font=\normalsize,#1]
    \begin{scope}[xshift=0cm]
      \fill[ps/phase] (-.5,.5) rectangle (3.5,-3.5);
      \draw[ps/stabline] (3.5,.5)--(3.5,-4.05);
      \node[anchor=base,font=\small\bfseries,text=black!60] at (1.5,.78) {stabilisation};
      \foreach \a/\b in {4/5,9/10}{
        \fill[ps/wave] (\a-.38,.42) rectangle (\b+.38,-2.42);
      }
      \foreach \r in {0,1,2}{
        \draw[ps/line] (-.5,-\r)--(10.5,-\r);
      }
      \draw[ps/line] (-.5,-3)--(2,-3);
      \draw[black!55,line width=.9pt,line cap=butt]
        (2,-3) +(-.17,-.17) -- +(.17,.17) +(-.17,.17) -- +(.17,-.17);
      \foreach \r/\p in {0/1,1/2,2/3,3/4}{
        \node[anchor=east] at (-.75,-\r) {$\p$};
      }
      \foreach \x/\r in {1/0,2/0,0/1,3/1,0/3,1/3}{
        \draw[ps/free] (\x,-\r-.27)--(\x,-\r+.27);
      }
      \foreach \x/\r in {4/0,9/0,5/1,10/1,4/2,10/2}{
        \draw[ps/stable] (\x,-\r-.27)--(\x,-\r+.27);
      }
      \node[anchor=base,font=\small\bfseries,text=psBlue] at (7,.78) {pulsing};
      \foreach \x in {4,5}{
        \draw[ps/guide] (\x,-2.42)--(\x,-2.9);
      }
      \draw[ps/dim] (4,-2.9)--(5,-2.9) node[midway,below=1pt] {$\le \sigma$};
      \draw[ps/dim] (5.38,-2.9)--(8.62,-2.9) node[midway,below=1pt] {$> \sigma$};
      \draw[black!60,line width=.6pt,-{Stealth[length=4pt,width=3.5pt]}]
        (-.5,-4.05)--(11,-4.05);
      \node[anchor=east] at (-.75,-4.05) {$t$};
      \foreach \x in {0,...,10}{
        \draw[black!60,line width=.6pt] (\x,-4.05)--(\x,-4.17);
      }
      \node[below] at (0,-4.17) {$0$};
      \node[below] at (4,-4.17) {$T$};
      \node at (5,-5.55) {(a) pulse synchronisation};
    \end{scope}
    \ccPanel{8.4cm}{(b) exact synchronous counting}
      {2,0,3,1}{1,1,0,0}{3,2,2,2}{0,3}
      {0,1,2,3,0,1,2}{0,1,2,3,0,1,2}{0,1,2,3,0,1,2}
  \end{tikzpicture}%
}

\newcommand{\CountingLiftFigure}[1][]{%
  \begin{tikzpicture}[x=.6cm,y=.6cm,line cap=round,font=\normalsize,#1,
    cc/reset/.style={fill=orange!18,rounded corners=2pt}]
    \foreach \a/\b in {5/6,8/8}{\fill[cc/reset] (\a-.38,.42) rectangle (\b+.38,-2.42);}
    \begingroup
    \renewcommand{\ccT}{3}\renewcommand{\ccLast}{12}%
    \ccPanel{0cm}{(a) outputs in $\Z_6$}
      {3,1,0}{2,4,1}{0,0,3}{4,2}
      {2,3,4,0,1,0,1,2,2,3}{3,4,4,0,1,0,2,2,2,3}{2,3,0,1,2,0,1,1,2,4}
    \endgroup
    \begin{scope}[xshift=9.4cm]
      \foreach \a/\b in {2/3,5/5}{\fill[cc/reset] (\a-.38,.42) rectangle (\b+.38,-2.42);}
      \draw[ps/stabline] (-.5,.5)--(-.5,-4.05);
      \node[anchor=base,font=\small\bfseries,text=psBlue] at (4.5,.78) {lift};
      \foreach \r/\p in {0/1,1/2,2/3,3/4}{
        \node[anchor=east] at (-.75,-\r) {$\p$};
      }
      \ccRow{0}{cc/stable}{0}{2,3,4,6,7,12,13,14,14,15}
      \ccRow{-1}{cc/stable}{0}{3,4,4,6,7,12,14,14,14,15}
      \ccRow{-2}{cc/stable}{0}{2,3,6,7,8,12,13,13,14,16}
      \draw[black!60,line width=.6pt,-{Stealth[length=4pt,width=3.5pt]}]
        (-.5,-4.05)--(10,-4.05);
      \node[anchor=east] at (-.75,-4.05) {$t$};
      \foreach \x in {0,...,9}{
        \draw[black!60,line width=.6pt] (\x,-4.05)--(\x,-4.17);
      }
      \node[below] at (0,-4.17) {$T$};
      \node at (4.5,-5.55) {(b) a $2$-lift};
    \end{scope}
  \end{tikzpicture}%
}

\newcommand{\PathCountingLiftFigure}[1][]{%
  \begin{tikzpicture}[x=.6cm,y=.6cm,line cap=round,font=\normalsize,#1,
    ac/node/.style={circle,draw=black!55,fill=white,line width=.8pt,
      minimum size=17pt,inner sep=0pt},
    ac/arc node/.style={ac/node,draw=psBlue,fill=psBlue,text=white}]
    \begin{scope}[shift={(0cm,-1.5)}]
      \def\acR{1.15cm}
      \draw[ps/stabline] (90:\acR-.42cm)--(90:\acR+.42cm);
      \pgfmathsetmacro{\acGap}{deg(9pt/\acR)}
      \foreach \k in {0,...,4}{
        \pgfmathsetmacro{\acA}{54-72*\k}
        \def\acEdge{black!55,line width=.8pt,-{Stealth[length=5pt,width=4.5pt]}}
        \ifnum\k=4 \def\acEdge{psBlue,line width=3pt,line cap=butt,-{Stealth[length=6pt,width=7pt]}}\fi
        \ifnum\k=0 \def\acEdge{psBlue,line width=3pt,line cap=butt,-{Stealth[length=6pt,width=7pt]}}\fi
        \expandafter\draw\expandafter[\acEdge] (\acA:\acR)
          arc[start angle=\acA,delta angle=-72+\acGap,radius=\acR];
      }
      \foreach \k in {0,...,4}{
        \pgfmathsetmacro{\acA}{54-72*\k}
        \def\acStyle{ac/node}
        \ifnum\k=0 \def\acStyle{ac/arc node}\fi
        \ifnum\k=1 \def\acStyle{ac/arc node}\fi
        \ifnum\k=4 \def\acStyle{ac/arc node}\fi
        \node[\acStyle] at (\acA:\acR) {$\mathbf{\k}$};
      }
    \end{scope}
    \node at (0cm,-5.55) {(a) a $2$-path};
    \begin{scope}[xshift=3.2cm]
      \fill[ps/wave] (5.62,.42) rectangle (6.38,-2.42);
    \end{scope}
    \begingroup
    \renewcommand{\ccT}{3}\renewcommand{\ccLast}{9}%
    \ccPanel{3.2cm}{(b) outputs}
      {3,1,0}{2,4,1}{0,0,3}{4,2}
      {2,3,4,0,1,2,3}{1,2,3,4,0,1,2}{3,4,0,1,2,3,4}
    \endgroup
    \begin{scope}[xshift=10.9cm]
      \draw[ps/stabline] (-.5,.5)--(-.5,-4.05);
      \node[anchor=base,font=\small\bfseries,text=psBlue] at (3,.78) {lift};
      \foreach \r/\p in {0/1,1/2,2/3,3/4}{
        \node[anchor=east] at (-.75,-\r) {$\p$};
      }
      \ccRow{0}{cc/stable}{0}{2,3,4,5,6,7,8}
      \ccRow{-1}{cc/stable}{0}{1,2,3,4,5,6,7}
      \ccRow{-2}{cc/stable}{0}{3,4,5,6,7,8,9}
      \draw[black!60,line width=.6pt,-{Stealth[length=4pt,width=3.5pt]}]
        (-.5,-4.05)--(7,-4.05);
      \node[anchor=east] at (-.75,-4.05) {$t$};
      \foreach \x in {0,...,6}{
        \draw[black!60,line width=.6pt] (\x,-4.05)--(\x,-4.17);
      }
      \node[below] at (0,-4.17) {$T$};
      \node at (3,-5.55) {(c) a $2$-lift};
    \end{scope}
  \end{tikzpicture}%
}

\newcommand{\ClockOffsetsFigure}{%
  \begingroup
  \WrapArcSetup{q=5,radius=1.3cm,cycle node size=17pt,value font=\normalsize,
    label font=\normalsize,node color=black!55,node width=.8pt,
    arc color=black!55,arc width=.8pt,directed edges=true,
    highlight color=psBlue,highlight width=3pt,selected fill=psBlue,
    selected width=.8pt,interior fill=psBlue,interior text=white,
    offset color=black!75,reverse color=black!75,
    cut color=black!55,cut width=.6pt,cut dash pattern={on 2.5pt off 2pt},
    cut length=8.4mm,offset outer radius=1.95cm,offset label gap=3pt,
    start label={},end label={},padding=.85cm,offset style=overlay}%
  \begin{tabular}{c@{\hspace{1.4cm}}c}
    \ClockOffsetCycle{4}{1} & \ClockOffsetCycle{2}{4} \\[2ex]
    (a) $a = 4$, $b = 1$ & (b) $a = 2$, $b = 4$
  \end{tabular}%
  \endgroup
}

\tikzset{
  oc/square/.style={
    os/advance/.append style={dashed,draw=black!45,line width=.9pt},
    os/advance i/.style={bend left=30},os/advance j/.style={bend right=30},
    os/offset/.style={gc/edge,gc/oriented}},
}
\newcommand{\OffsetConsistencyFigure}{%
  \begin{tabular}{c@{\hspace{2.2cm}}c}
  \OffsetSquare[show lifts=false,width=3.2cm,height=1.6cm,round gap=1.15cm,
    baseline={(0,.5)},advance color=black!70,offset color=black!70,
    tikz={oc/square,os/first/.style={gc/node,gc/a,inner sep=3pt},
      os/second/.style={gc/node,gc/b,inner sep=3pt},
      os/process label/.style={overlay}},
    corner 1={\phi(i,T)}, corner 2={\phi(i,T+1)},
    corner 3={\phi(j,T)}, corner 4={\phi(j,T+1)},
    advance i=\Delta(y_i), advance j=\Delta(y_j),
    offset T={D(\prefix{y_i},\prefix{y_j})},
    offset T+1={D(\suffix{y_i},\suffix{y_j})}]{0}{0}{0}{0}
  &
  \OffsetSquare[show lifts=false,q=5,width=2.4cm,height=1.6cm,round gap=1.15cm,
    baseline={(0,.5)},advance color=black!70,offset color=black!70,
    tikz={oc/square,os/first/.style={gc/node,gc/a},os/second/.style={gc/node,gc/b}},
    corner 1=\mathbf{4},corner 2=\mathbf{0},corner 3=\mathbf{0},corner 4=\mathbf{2},
    first process={},second process={}]{4}{5}{5}{7}
  \\[2ex]
  (a) & (b)
  \end{tabular}%
}


